Correct-by-Design Control of Parametric Stochastic Systems

This paper addresses the problem of computing controllers that are correct by design for safety-critical systems and can provably satisfy (complex) functional requirements. We develop new methods for models of systems subject to both stochastic and parametric uncertainties. We provide for the first time novel simulation relations for enabling correct-by-design control refinement, that are founded on coupling uncertainties of stochastic systems via sub-probability measures. Such new relations are essential for constructing abstract models that are related to not only one model but to a set of parameterized models. We provide theoretical results for establishing this new class of relations and the associated closeness guarantees for both linear and nonlinear parametric systems with additive Gaussian uncertainty. The results are demonstrated on a linear model and the nonlinear model of the Van der Pol Oscillator.

==> Gaussplot.tex <==
%\begin{figure}[htp]
%%\pgfmathdeclarefunction{dnorm}{2}{%
%%	\pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
%%}
%
%\begin{tikzpicture}
%	\begin{axis}[
%		domain=0:9,
%		samples=101,
%		height=5cm,
%		width=10cm
%		]
%		
%		% Fill aread under both curves, start stacking
%		\addplot [
%		fill=yellow,
%		draw=none,
%		domain=0:10,
%		stack plots=y
%		] {min(dnorm(4,1),dnorm(5,1)) } \closedcycle;
%	
%
%		% Draw curves
%		\addplot [thin, smooth, name path global=first] {dnorm(4,1)};
%		\addplot [thin, smooth, name path global=second] {dnorm(4,1)};
%
%	\end{axis}
%\end{tikzpicture}
%\caption{Computation of $\Wt$ given $\hat \Tr$ and $\Tr$. }\label{fig:Comp_W}
%\end{figure}

\begin{figure}
\begin{tikzpicture} 
	
	\begin{axis}[samples=150,
		domain=0:10,clip = false,
		xlabel={$\xhp$},
		zmin=0,
%		zlabel={$p(\cdot)$},
		zlabel={$t(d\xp)$},
		samples y=0, ylabel={$\xp$},
		area plot/.style={
			fill opacity=0.45,
			draw=none,
			fill=blue!70,
			mark=none,
			smooth
		}
		]\addplot3[blue, mark=none, smooth, style=semithick, densely dashed]  (x,x,{min(dnorm(4,1),dnorm(5,1)) });	
		\addplot3 [area plot] (x,x,{min(dnorm(4,1),dnorm(5,1)) });	
		\draw [black, densely dotted, style=thin] (axis cs: 0,5,0) -- (axis cs: 0,5,0.4);
		\draw [black, densely dotted, style=thin] (axis cs: 0,5,0) -- (axis cs: 5,5,0);
		\addplot3 [blue, mark=none, smooth, style=semithick, densely dashed] (0,x,{min(dnorm(4,1),dnorm(5,1)) });
		\addplot3 [black, mark=none, smooth, style=semithick]  (0,x,{dnorm(5,1) });
		\addplot3 [area plot] (0,x,{min(dnorm(4,1),dnorm(5,1)) });
		\draw (0,0) -- (6,0) -- (6,3) -- (0,3) -- cycle;
		\node (A) at (axis cs: 5,10,0.4) [red, right] {$\theta$};
		\draw [red, solid, style=semithick] (axis cs: 4,10,0.4) -- (axis cs: 5,10,0.4);
		\draw [red, densely dotted, style=thin] (axis cs: 4,10,0) -- (axis cs: 4,10,0.4);
		\draw [black, densely dotted, style=thin] (axis cs: 5,10,0) -- (axis cs: 5,10,0.4);
		\draw [black, densely dotted, style=thin] (axis cs: 5,10,0) -- (axis cs: 5,5,0);
		\addplot3 [blue, mark=none, smooth, style=semithick, densely dashed] (x,10,{min(dnorm(4,1),dnorm(5,1)) });
		\addplot3 [black, mark=none, smooth, style=semithick]  (x,10,{dnorm(4,1) });
		\addplot3 [area plot] (x,10,{min(dnorm(4,1),dnorm(5,1)) });
		\node (B) at (axis cs: 11,10,0.12) [black, right, rotate = 90] {$\hat t(d\xhp)$};
%		\node (C) at (axis cs: 0,6,0.2) [black, right, rotate = 30] {$t(d\xp)$};
		\node (C) at (axis cs: 6,3.5,0) [blue, rotate = 5] {$v(d\xhp\times d\xp)$};
		


%		\addplot3 [area plot] (x,9,{normal(20,1)});
%		\addplot3 [area plot] (x,8,{normal(20,1)});
%		\addplot3 [area plot] (x,7,{normal(20,1)});
	\end{axis}
\end{tikzpicture}
\caption{Two dimensional representation of the computation of $\W$ for some $\xh{},\x{},\ach{}$ given the evaluated stochastic transition kernels $\hat t$ and $t$.  \Oliver{Use this figure in the main body of the journal paper version.}}\label{fig:Comp_W}
\label{fig:gaussplot}
\end{figure}

==> compositional.tex <==
% !TEX root = main_cdc_22.tex
\begin{comment}
\color{gray}
\section{Compositional approach for sub-probability couplings of subsystems}
%\begin{quote}
%	"The abstraction framework is based on the notion of $\delta$-lifted relations, using which one can quantify the distance in probability between the interconnected gMDPs and that of their abstractions." \cite{lavaei2021compositional}
%\end{quote}
\Oliver{Insert short introduction with reference to \cite{lavaei2021compositional}.}\\
In the following, we drop the index $k$ on the time series $x_k,u_k$ for brevity.
Consider multiple interconnected gMDPs $\M_i$, $i=1,\ldots,N$, with unknown parameters $\theta_i\in\Theta_i$, respectively:
\begin{align}
	\M_i(\theta_i): \left\{ \begin{array}{ll}
		\xp_i &= f_i(x_i,(u_i,v_i);\theta_i)+ R_i w_i\\
		y_i &= h_i(x_i),
	\end{array} \right.\label{eq:nonlinear_sys_subsys}
\end{align}
where $v_i$ denotes the internal inputs of subsystem $i$.
The nominal models are given as
\begin{align}
	\Mh_i: \left\{ \begin{array}{ll}
		\xhp_i &= \hat f_i(\hat x_i, (\hat u_i, \hat v_i);\theta^0_i)+ R_i\hat w_i\\
		\hat y_i &=  \hat h_i( \hat x_i).
	\end{array} \right.\label{eq:nonlinear_nom_subsys}
\end{align}
Note that the outputs $y_{ii}$, where $y_i:=[y_{i1},\ldots,y_{iN}]\T$, are external outputs, while $y_{ij}$ with $i\neq j$ are used internally to connect the individual subsystems to one another.

In the following, we assume that for all subsystems $i=1,\ldots,N$ we have \mbox{$\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i$} and derive conditions so that \mbox{$\Mh\preceq^{\delta}_\eps\M$}, where $\Mh$ and $\M$ are the interconnections of their respective subsystems. In the following, we formalize these concepts mathematically. First, we extend the definition of an SSR as stated in Def.~\ref{def:subsim} to subsystems.
\begin{definition}[SSR for subsystems]\label{def:ssr_subsys}
%	\Oliver{Replacement for Def.~3.2 in \cite{lavaei2021compositional}.}
	Consider two gMDPs
	$\M\!=\!(\X,x_0,\A\times\V, \Tr, h, \Y)$ and $\Mh\!=\!(\Xh,\xh{0},\Ah\times\Vh, \Trh, \hat h,  \Y)$, measurable relations $\R_{x}\subset \Xh\times\X$ and \Oliver{$\R_{\iin{}}\subset \Vh\times\V$}, and an interface function \(\InF :\Xh\times\X\times\Ah \rightarrow \A\). If there exists a sub-probability kernel  $\Wt(\cdot|\xh{},x, \Oliver{(\uh{}, \hat v, v)})$
such that
\begin{itemize}\itemsep=0pt
	\item[(a)] $(\hat x_{0}, x_{0})\in \R_{x}$;
	\item[(b)] for all $(\hat x,x)\in\R_{x}$, all $(\hat v,v)\in\R_{\iin{}}$, and $\ach{}\in \Ah$, $\Wt(\cdot|\xh{},x, \Oliver{(\uh{}, \hat v, v)})$ is a sub-probability coupling  of $\hat \Tr(\cdot|\hat x,\Oliver{(\uh{}, \hat v)})$ and $\Tr(\cdot|x,\Oliver{(\InF, v)})$ over $\R_{x}$ with respect to $\delta$ (c.f. Def.~\ref{def:submeasure_lifting}),
	\item[(c)] $\forall (\hat x,x)\in\R_{x}: \mathbf d_\Y(\hat h(\hat x),h(x)) \leq \varepsilon$,
\end{itemize}
then $\Mh$ is in an $(\varepsilon,\delta)$-SSR with $\M$  that is denoted as \mbox{$\Mh\preceq^{\delta}_\eps\M$}.
\end{definition}

%\begin{definition}[\bfseries Closeness for a composed system]\label{thm:closeness_composition}
%	\Oliver{Replacement for Thm.~3.5 in \cite{lavaei2021compositional}. Necessary?}
%\end{definition}
Let $\M_i\!=\!(\X_i,x^0_i,\A_i\times\V_i, \Tr_i, h_i, \Y_i)$ be a gMDP.
We can partition the internal input and output of $\M_i$ as
\begin{equation}\label{eq:partion_inout}
	v_i = [v_{i1}\T;\ldots;v_{i(i-1)}\T;v_{i(i+1)}\T;\ldots;v_{iN}\T], \quad i=1,\ldots,N,
\end{equation}
and the output space and function such that
\begin{equation}\label{eq:partion_infcn}
	h_i(x_i) = [h_{i1}\T(x_i);\ldots;h_{iN}\T(x_i)], \quad \Y_i=[\Y_{i1};\ldots;\Y_{iN}].
\end{equation}
%\begin{equation*}
%	C_i = [c_{i1}\T;\ldots;c_{iN}\T], \quad \Y_i=\Oliver{\bigcup_{j=1}^{N}}\Y_{ij}. \Oliver{\text{ or product?}}
%\end{equation*}
Furthermore, we separate the internal outputs $y_{ij}$, where $i\neq j$, from the external ones, i.e., $y_{ii}$, by forming interconnection constraint maps $g_i$, which will facilitate the interconnection of multiple gMDPs by enforcing $v_{i}=g_{i}$:
\begin{align}
	\begin{split}\label{eq:interconnection_constraint_maps}
		g_i(x_1,\ldots,x_N):=[h_{1i}\T (x_1);\ldots;h_{(i-1)i}\T (x_{i-1});\\h_{(i+1)i}\T (x_{i+1});\ldots;h_{Ni}\T (x_N)].
	\end{split}
\end{align}
Next, we define the interconnection of multiple subsystems.

\begin{definition}[Interconnection of subsystems]\label{def:interconnection}
%	\Oliver{Replacement for Def.~4.1 in \cite{lavaei2021compositional}.}
	Consider $N\in\mathbb{N}_{\geq 1}$ gMDPs $\M_i\!=\!(\X_i,x^0_i,\A_i\times\V_i, \Tr_i, h_i, \Y_i)$, $i=1,\ldots,N$, with an input-output configuration which can be partitioned as in \eqref{eq:partion_inout}-\eqref{eq:partion_infcn}. Then, the \emph{interconnection} of subsystems $\M_i$ is a gMDP $\M\!=\!(\X,x^0,\A\times\V, \Tr, h, \Y)$, also denoted as $\Interc{\M_1,\ldots,\M_N}$, such that $\X=[\X_{1};\ldots;\X_{N}]$, $\U=[\U_{1};\ldots;\U_{N}]$, $\V=[\V_{1};\ldots;\V_{N}]$, $\Y=[\Y_{11};\ldots;\Y_{NN}]$, $h=[h_{11};\ldots;h_{NN}]$, with interconnection constraints
	\begin{equation}\label{eq:interconnection_constraints}
		\forall i,j=1\ldots,N,\, i\neq j:\, v_{ji}=y_{ij},\, \Y_{ij}\subseteq\V_{ji}.
	\end{equation}
	The kernel and initial distribution are given as $\Tr=\prod_{i=1}^{N}\Tr_{i}$ and $x^0=[x^0_{1};\ldots;x^0_{N}]$, respectively.
\end{definition}

In the next theorem we establish \mbox{$\Mh\preceq^{\delta}_\eps\M$}, where $\M=\Interc{\M_1,\ldots,\M_N}$ and $\Mh=\Interc{\Mh_1,\ldots,\Mh_N}$, by induction from $\forall i=1,\ldots,N:\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i$.

\begin{theorem}[\bfseries Induced compositional SSR]\label{thm:comp_induction}
%	\Oliver{Replacement for Thm.~4.3 in \cite{lavaei2021compositional}.}
	Consider $N\in\mathbb{N}_{\geq 1}$ gMDPs $\M_i(\theta_i)$, $i=1,\ldots,N$, forming an interconnected gMDP $\M(\theta)=\Interc{\M_1,\ldots,\M_N}$, with $\theta:=[\theta_1,\ldots,\theta_N]$. Suppose that there exist $N$ abstract gMDPs $\Mh_i$ independent of $\theta_i$, such that for all $i=1,\ldots,N$ $\Mh_i$ is in an $(\varepsilon_i, \delta_i)$-SSR with $\M_i(\theta_i)$ as defined in Def.~\ref{def:ssr_subsys} with corresponding relations $R_{x_i}$, $\R_{\iin{i}}$, and sub-probability coupling $\Wt_i$. If for all \red{$i,j=1,\ldots,N$ we have
	\begin{equation*}
		\forall (\hat x_j, x_j)\in\R_{x_j}: \, \left(\hat g_i(\hat x_1,\ldots,\hat x_N), g_i(x_1,\ldots,x_N)\right)\in\R_{\iin{i}},
	\end{equation*}
	}with interconnection constraint maps $\hat g_i$, $g_i$ as defined in \eqref{eq:interconnection_constraint_maps},
	then $\Mh=\mathscr{I}(\Mh_1,\ldots,\Mh_N)$ is in an \emph{induced compositional} $(\varepsilon, \delta)$-SSR with $\M(\theta)$ as defined in Def.~\ref{def:subsim} with a relation $\R$ given as 
	\begin{equation*}
		(\hat x, x)\in\R \Leftrightarrow \forall i=1,\ldots,N:\, (\hat x_i, x_i)\in\R_{x_i}
	\end{equation*}
	where $\hat x:=[\hat x_1;\ldots;\hat x_N]$ and $x:=[x_1;\ldots;x_N]$,
	and \Oliver{$\varepsilon=\sum_{i=1}^{N}\varepsilon_i$}, \Oliver{$\delta=1-\prod_{i=1}^{N}(1-\delta_i)$}. Furthermore, we obtain the sub-probability coupling \Oliver{$\Wt=\prod_{i=1}^{N}\Wt_{i}$} and the interface function \Oliver{$\InF=\prod_{i=1}^{N}\InF_{i}$}, substituting with the interconnection constraints in \eqref{eq:interconnection_constraints}.
\end{theorem}


\subsection{Linear subsystems}
Let us now look at the case where the overall system can be decomposed into multiple linear subsystems $\M_i$. 
Consider $N$ interconnected gMDPs, $i=1,\ldots,N$, i.e.,
\begin{align}
	\M_i(\theta_i): \left\{ \begin{array}{ll}
		\xp_i &= A_i x_i+ B_i u_i+ D_i v_i+ R_i w_i+F_i \theta_i\\
		y_i &= C_i x_i,
	\end{array} \right.\label{eq:linear_sys_subsys}
\end{align}
and corresponding nominal models
\begin{align}
	\Mh_i: \left\{ \begin{array}{ll}
		\xhp_i &= A_i \hat x_i+  B_i \hat u_i+ D_i \hat v_i+ R_i\hat w_i\\
		\hat y_i &=  C_i \hat x_i.
	\end{array} \right.\label{eq:linear_nom_subsys}
\end{align}
%Note that the outputs $y_{ii}$, where $y_i:=[y_{i1},\ldots,y_{iN}]\T$, are external outputs, while $y_{ij}$ with $i\neq j$ are used internally to connect the individual subsystems to each other.
The transition kernels can consequently be written as
\begin{align*}
	\Tr_i(\dxp_i \given x_i, u_i, v_i) &= \mathcal N(\dxp_i|A_i x_i+ B_i u_i+ D_i v_i +F_i \theta_i, R_iR_i\T)\\
	\Trh_i(\dxhp_i \given \hat x_i, \hat u_i, \hat v_i) &= \mathcal N(\dxhp_i|A_i \hat x_i+ B_i \hat u_i+ D_i \hat v_i, R_iR_i\T).
\end{align*}

%\hrule
We choose the interface function $\ac{i}\sim\InF_i(\cdot|\hat x_i, x_i, \hat u_i):=\ach{i}$,
and the noise coupling $\hat w_i=w_i+R^{-1}_i F_i\theta_i$ to get the state mapping
\[ \xhp_i = \xp_i-A (x_i-\hat x_i)-B (\ac{i}-\ach{i})-D(v_i-\hat v_i), \]
not dependent on $\theta$, i.e.,
\begin{equation}
	\label{eq:statemap_subsys}
	\xhp_i \sim \Refi_i(\cdot |\xh{i}, \x{i}, \xp_{i},\ach{i}) = \delta_{\xp_i-A x^\Delta_i-B u^\Delta_i-Dv^\Delta_i}(d\xhp_i),
\end{equation}
where $v^\Delta_i:=v_{i}-\hat v_{i}$.
To establish an SSR $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$, we select the relations
\begin{align}
	\R_{x_i}&:=\{ (\hat x_i,x_i)\in\Xh_i\times\X_i \given x_i=\hat x_i\}\label{eq:R_x}\\
	\R_{\iin{i}}&:=\{ (\hat v_i,v_i)\in\Vh_i\times\V_i \given v_i=\hat v_i\}.\label{eq:R_v}
\end{align}
Condition (a) of Def.~\ref{def:ssr_subsys} holds by setting the initial states $\hat x^{0}_i = x^{0}_i$. Condition (c) is satisfied with $\eps_i=0$ since both systems use the same output mapping. For condition (b), we define the sub-probability coupling $\Wt_i$ of $\hat \Tr_i(\cdot|\hat x_i,\ach{i})$ and $\Tr_i(\cdot|x_i,\InF_i)$ over $\R_{x_i}$:
\begin{align}
	\begin{split}\label{eq:subprobcoup_subsys}
		\Wt_i
		&=\del{d\xhp_i}{\xp_i}
		\min\{\mathcal N(d\xp_i|\Phi_i,R_iR_i\T),\\&\mathcal N(d\xp_i|\Phi_i-R^{-1}_i F_i\theta_i, R_iR_i\T)\},
	\end{split}
\end{align}
with $\Phi_i := A_i x_i+ B_i u_i+ D_i v_i+ F_i\theta_i$, that takes the minimum of two probability measures.

\begin{theorem}
	\label{thm:linear_subsys}
	For the linear models in \eqref{eq:linear_sys_subsys}-\eqref{eq:linear_nom_subsys}, we have that $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$ with interface function $\ac{i} = \ach{i}$, relations \eqref{eq:R_x}-\eqref{eq:R_v}, and the sub-probability kernel \eqref{eq:subprobcoup_subsys}. The state mapping \eqref{eq:statemap_subsys} defines a valid control refinement with $\eps_i=0$ and
	\begin{equation}
		\label{eq:delta_subsys}
		\delta_i = \sup_{\theta_i\in\Theta_i}\left\lbrace  1 - 2\cdot\cdf{-\frac{1}{2}\norm{R^{-1}_i F_i\theta_i}}\right\rbrace.
	\end{equation}
\end{theorem}

	
\subsection{\Oliver{Composed system}}
Now we connect two subsystems, $i\in\{1,2\}$, with $\iin{1}=y_2$ and $\iin{2}=y_1$ (i.e., with $\iinh{1}=\hat y_2$ and $\iinh{2}=\hat y_1$). For $x:=[x_1,x_2]\T\in\X$, $\hat x:=[\hat x_1,\hat x_2]\T\in\Xh$, $u:=[u_1,u_2]\T\in\A$, $\hat u:=[\hat u_1,\hat u_2]\T\in\Ah$, and $\theta:=[\theta_1,\theta_2]\T\in\Theta$ we find the compositional transition kernels for the interconnected gMDPs $\M(\theta)$ and $\Mh$, namely
\begin{align*}
	\Tr(\dxp \given x, u) &= \mathcal N(\dxp|\bar A x+ B u+F \theta, RR\T)\\
	\Trh(\dxhp \given \hat x, \hat u) &= \mathcal N(\dxhp|\bar A \hat x+ B \hat u, RR\T).
\end{align*}
%with $u=\hat u$, $x=\hat x$, and 
where $B:=\mathrm{diag}(B_1,B_2)$, $F:=\mathrm{diag}(F_1,F_2)$, $R:=\mathrm{diag}(R_1,R_2)$, and
\begin{align*}
	\bar A&:=\begin{bmatrix} A_1 & D_1C_2 \\ D_2C_1 & A_2 \end{bmatrix}.
\end{align*}

We get the state mapping
\[ \xhp = \xp-\bar A (x-\hat x)-B (\ac{}-\ach{}), \]
not dependent on $\theta$, i.e.,
\begin{equation}
	\label{eq:statemap_comp}
	\xhp \sim \Refi(\cdot |\xh{}, \x{}, \xp{},\ach{}) = \delta_{\xp-\bar A x^\Delta-B u^\Delta}(d\xhp).
\end{equation}
To establish an SSR of the composed system, i.e., $\Mh\preceq^{\delta}_{\eps}\M(\theta)$, we select the relation
\begin{align}\label{eq:R_comp}
	\R_{x}&:=\{ (\hat x,x)\in\Xh\times\X \given x=\hat x\}
\end{align}
Condition (a) of Def.~\ref{def:subsim} holds by setting the initial states $\hat x^{0} = x^{0}$. Condition (c) is satisfied with $\eps=0$ since both compositional systems use the same output mapping, i.e., $C:=\mathrm{diag}(C_1,C_2)$. For condition (b), we define the sub-probability coupling $\Wt$ of $\hat \Tr(\cdot|\hat x,\ach{})$ and $\Tr(\cdot|x,\InF)$ over $\R_{x}$:
\begin{align}
	\begin{split}\label{eq:subprobcoup_comp}
		\Wt&=\del{d\xhp}{\xp} \min\{\mathcal N(d\xp|\Phi,RR\T),\\
		&\mathcal N(d\xp|\Phi-R^{-1}F\theta_, RR\T)\},
	\end{split}
\end{align}
with $\Phi := \bar A x+ B u+ F\theta$, that takes the minimum of two probability measures.

Now we want to establish a probabilistic relation after the composition using Thm.~\ref{thm:comp_induction}, which enables us to get guarantees on the closeness of the composed system and its abstraction using Thm.~\ref{thm:linear_subsys}.

%\subsection{\Oliver{Establishing probabilistic relations}}
%In this subsection, we derive the conditions under which $\Mh$ in \eqref{eq:linear_nom_subsys} is in an $(\varepsilon,\delta)$-SSR with $\M$ in \eqref{eq:linear_sys_subsys} with relations $\R_x$ and $\R_w$ as defined in \eqref{eq:R_x}-\eqref{eq:R_v}.

\begin{theorem}
	Consider $N\in\mathbb{N}_{\geq 1}$ linear subsystems \eqref{eq:linear_sys_subsys}-\eqref{eq:linear_nom_subsys}, where $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$ for $i=1,\ldots,N$ with relations \eqref{eq:R_x}-\eqref{eq:R_v}, interface functions $u_i=\hat u_i$, and sub-probability kernels \eqref{eq:subprobcoup_subsys}.
	Let, $\M=\Interc{\M_1,\ldots,\M_N}$ and $\Mh=\Interc{\Mh_1,\ldots,\Mh_N}$ be the interconnections of these linear subsystems. Then Thm.~\ref{thm:comp_induction} holds, with relation $\R=\{ (\hat x,x)\in\Xh\times\X\given x=\hat x\}$, interface function $\ac{} = \ach{}$, and sub-probability kernel \eqref{eq:subprobcoup_comp}.
\end{theorem}
\begin{proof}
	It is trivial to show that the interconnection constraints in Thm.~\ref{thm:comp_induction} hold for this choice of $\R_{x_i},\R_{\iin{i}}$.
\end{proof}


%
%	\Oliver{
%		Using $\hat w:= \Gamma w+\offset$
%		\subsubsection{Def.~\ref{def:submeasure_lifting}(a)}\label{app:def_sub_a}
%		To prove that all considered distributions of \eqref{eq:subprobcoup_new} satisfy $\operatorname{supp}(\W)\subset\rel$ (c.f. Def.~\ref{def:submeasure_lifting}(a)), we first show $\forall z\in\Z: \W(\Xh\times\X)\geq 1-\delta$ and then $\forall z\in\Z: \W(\Xh\times\X) = \W(\R)$.
%		
%		
%		From Eq.~\eqref{eq:subprobcoup_new} we get for a fixed $z\in\Z$
%		\begin{align*}
%			&\W(\Xh\times\X) = \int_{\xhp\in\Xh} \int_{\xp\in\X} \int_{w} \W(\dxhp\times \dxp)\\
%			&= \int_{w} \int_{\xhp\in\Xh} \int_{\xp\in\X} \fhdel{\dxhp| \Gamma w+\offset} \fdel{\dxp| w; \theta} \\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}.
%		\end{align*}
%		Using definitions \eqref{eq:fdel_lin_new}-\eqref{eq:fhdel_lin_new} we rewrite to obtain
%		\begin{align*}
%			&\W(\Xh\times\X) = \int_{w} \int_{\xhp\in\Xh} \int_{\xp\in\X} \delta_{\hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)}(\dxhp)\\
%			&\delta_{Ax_k+Bu_k+Rw+F\theta}(\dxp) \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}\\
%			&= \int_{w} \1(A x_k+B u_k+Rw+F\theta\in\X)\\& \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)\in\Xh)\\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}.
%		\end{align*}
%		Since $\forall z\in\Z,w\exists\xp\in\X: \xp = A x_k+B u_k+Rw+F\theta$ and $\forall z\in\Z,w\exists\xhp\in\Xh: \xhp = \hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)$, we get $\W(\Xh\times\X) = \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}$.
%		
%		
%		Similarly, we derive from \eqref{eq:subprobcoup_new}
%		\begin{align*}
%			&\W(\R) = \int_{(\xhp, \xp)\in\R} \int_{w} \W(\dxhp\times \dxp)\\
%			&= \int_{w} \int_{(\xhp, \xp)\in\R} \fhdel{\dxhp| \Gamma w+\offset} \fdel{\dxp| w; \theta} \\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}\\
%			&= \int_{w} \1((\hat A\hat x_k+\hat B\hat u_k+\Gamma w+\offset,\\&Ax_k+Bu_k+Rw+F\theta)\in\R)\\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\},
%			%	&= \int_{w} \int_{(\xhp, \xp)\in\R}  \delta_{f(\hat x_k,\hat u_k,w+\theta;\theta_0)}(\dxhp)\delta_{f(x_k,u_k,w;\theta)}(\dxp)\\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\theta, I)\}\\\
%		\end{align*}
%		and get after simplifying using $\hat x_k=x_k$ and $\ach{k}=\ac{k}$
%		\begin{align*}
%			&\W(\R) = \1((\hat A-A)\hat x_k+(\hat B-B)\hat u_k+(\Gamma-R) w+\offset=F\theta)\\& \int_{w}  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\},
%		\end{align*}
%		yielding $\W(\R) = \W(\Xh\times\X)$ independent of $z$. This proves that \eqref{eq:subprobcoup_new} satisfies condition (a) of Def.~\ref{def:submeasure_lifting}.
%		
%		
%		CALCULATION OF DELTA SKIPPED:
%		\begin{equation*}
%			\delta(\xh{k},\ach{k}) = \sup_{\theta\in\Theta}\left\lbrace  1 - 2\cdot\cdf{-\frac{1}{2}\Phi\norm{\offset(\xh{k},\ach{k},\theta)}}\right\rbrace
%		\end{equation*}
%		
%		\subsubsection{Def.~\ref{def:submeasure_lifting}(b)}\label{sec:proof_th3b_}
%		Prove $\forall z\in\Z,S \subset \hat \X:\W(S \times \X) \leq \hat t(S)$.
%		First, we consider the integral of the individual distributions of the transition kernel \eqref{eq:tr_hat_new} over $S$. For a fixed $z\in\Z$ we get
%		\begin{align}
%			\begin{split}\label{eq:transKernelTemp1_}
%				&\hat t(S) = \int_{\xhp\in S} \hat t(\dxhp) \\
%				&= \int_{\xhp\in S}  \int_{\hat w}\fhdel{\dxhp|\hat w}\mathcal N(d\hat w|0, I)\\
%				&=  \int_{\hat w} \int_{\xhp\in S} \delta_{\hat A\hat x_k+\hat B\hat u_k+\hat R\hat w}(\dxhp)\mathcal N(d\hat w|0, I)\\
%				&=  \int_{\hat w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat R\hat w \in S)\mathcal N(d\hat w|0, I).
%			\end{split}
%		\end{align}
%		We will use this equation later on. Next, from \eqref{eq:subprobcoup_new} we get
%		\begin{align*}
%			&\W(S \times \X) = \int_{\xhp\in S}  \int_{\xp\in \X}  \int_{w} \W(\dxhp \times \dxp)\\
%			&=  \int_{w}  \int_{\xp\in \X}  \fdel{\dxp| w; \theta} \int_{\xhp\in S} \fhdel{\dxhp| \Gamma w+\offset} \\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}\\
%			&=  \int_{w}  \int_{\xp\in \X} \delta_{Ax_k+Bu_k+Rw+F\theta}(\dxp)\\& \int_{\xhp\in S} \delta_{\hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)}(\dxhp)\\&  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}\\
%			&=  \int_{w} \1(A x_k+B u_k+Rw+F\theta\in\X)\\& \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)\in S)\\&  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}.
%		\end{align*}
%		Since $\forall z\in\Z,w \exists \xp\in \X: \xp = A x_k+B u_k+Rw+F\theta$, this integral can equivalently be written as
%		\begin{align*}
%			&\W(S \times \X) = \int_{w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(\hat R w+\offset)\in S)\\&  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\theta, I)\}\\
%			&= \int_{\hat w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(\hat R w+\offset)\in S)\\& \min\{ \frac{dw}{ \sqrt{(2\pi)^n \!\left| I \right| }}\exp\!\left[\!-\frac{1}{2}w\T\! I^{-1}\!w\!\right],\\& \frac{dw}{ \sqrt{(2\pi)^n \!\left| I \right| }}\exp\!\left[\!-\frac{1}{2}(w\!+\!\offset)\T\! I^{-1}\!(w\!+\!\offset)\!\right]\}\\
%			&= \int_{\hat w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat Rw\in S)\\& \min\{ \frac{dw}{ \sqrt{(2\pi)^n \!\left| \hat R\hat R\T \right| }}\exp\!\left[\!-\frac{1}{2}(w-\gamma)\T\! (\hat R\hat R\T)^{-1}\!(w-\gamma)\!\right],\\& \frac{dw}{ \sqrt{(2\pi)^n \!\left| \hat R\hat R\T \right| }}\exp\!\left[\!-\frac{1}{2}w\T\! (\hat R\hat R\T)^{-1}\!w\!\right]\}\\
%			&=\int_{w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat w\in S)\\&  \min\{\mathcal N(dw|\offset,\hat R\hat R\T),\mathcal N(dw|0,\hat R\hat R\T )\}\\
%			&= \int_{\hat w}  \1(\hat A\hat x_k+\hat B\hat u_k+\hat R\hat w\in S)\\&  \min\left\lbrace \mathcal N(d\hat w|\offset,I), \mathcal N(d\hat w|0,I)\right\rbrace\\
%			&\leq \int_{\hat w}  \1(A\hat x_k+B\hat u_k+\hat R\hat w\in S) \mathcal N(d\hat w|0,I).
%		\end{align*}
%		Substituting Eq.~\eqref{eq:transKernelTemp1__new} yields $\forall z\in\Z:\W(S \times \X) \leq  \hat t(S)$,
%		concluding that \eqref{eq:subprobcoup_new} satisfies condition (b) of Def.~\ref{def:submeasure_lifting}.
%		
%		\subsubsection{Def.~\ref{def:submeasure_lifting}(c)}
%		Prove $\forall z\in\Z,S \subset \X:\W(\Xh \times S) \leq t(S)$.
%		Analogously to App.~\ref{sec:proof_th3b__new} we consider the integral of the individual distributions of the transition kernel \eqref{eq:tr_new} over $S$. For a fixed $z\in\Z$ we get
%		\begin{align}
%			\begin{split}\label{eq:transKernelTemp2_}
%				&t(S) = \int_{\xhp\in S}t(\dxp) \\
%				&= \int_{w} \1(Ax_k+Bu_k+Rw+F\theta\in S)\mathcal N(dw|0, I).
%			\end{split}
%		\end{align}
%		Next, using Eq.~\eqref{eq:subprobcoup_new} we get
%		\begin{align*}
%			&\W(\Xh \times S) = \int_{\xhp\in \Xh}  \int_{\xp\in S}  \int_{w} \W(\dxhp \times \dxp)\\
%			&=  \int_{w}  \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(w+\theta)\in\Xh)\\ &\1(Ax_k+Bu_k+w+\theta\in S)\\&  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\theta, I)\}.
%		\end{align*}
%		Since $\forall z\in\Z,w \exists \xhp\in \Xh: \xhp = \hat A\hat x_k+\hat B\hat u_k+\hat R(w+\theta)$, it follows that
%		\begin{align*}
%			&\W(\Xh \times S) = \int_{w} \1(Ax_k+Bu_k+Rw+F\theta\in S)\\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\theta, I)\}\\
%			&\leq \int_{w} \1(Ax_k+Bu_k+Rw+F\theta\in S) \mathcal N(dw|0,I)\\
%			&= t(S),
%		\end{align*}
%		yielding $\forall z\in\Z:\W(\Xh \times S) \leq  t(S)$,
%		therefore concluding that \eqref{eq:subprobcoup_new} satisfies condition (c) of Def.~\ref{def:submeasure_lifting}. Hence, having proven that \eqref{eq:subprobcoup_new} satisfies all conditions of Def.~\ref{def:submeasure_lifting}, \eqref{eq:subprobcoup_new} is a valid sub-probability coupling.
%		
%		\subsubsection{Def.~\ref{def:validrefinement}}
%		From the state mapping $\hat R\hat w=Rw+F\theta$, i.e., $\xhp- \hat A\hat x-\hat B\hat u=\xp-Ax-Bu$, we find a composed probability measure using Eq.~\ref{eq:compprobmeas_new}:
%		\begin{align*}
%			&\bar{\Refi} = \delta_{\xp-Ax-Bu+\hat A\hat x+\hat B\hat u}(d\xhp) \Tr(\dxp|x,\InF(\ac{k}|\hat x_k, x_k, \hat u_k))\\
%			&= \delta_{\xp-Ax-Bu+\hat A\hat x+\hat B\hat u}(d\xhp) \int_w \fdel{\dxp|w;\theta} \mathcal N(dw|0, I)\\
%			&= \int_w \delta_{A\hat x_k+B\hat u_k+F\theta+Rw)}(d\xhp)  \fdel{\dxp|w;\theta} \mathcal N(dw|0, I)\\
%			&= \int_w \fhdel{\dxhp|\hat R^{-1}(F\theta+Rw)} \fdel{\dxp|w;\theta} \mathcal N(dw|0, I)\\
%			&= \int_w \int_{\hat w} \fhdel{\dxhp|\hat w} \fdel{\dxp|w;\theta}  \delta_{\hat R^{-1}(F\theta+Rw)}(d\hat w) \mathcal N(dw|0, I),
%		\end{align*}
%		which upper-bounds the sub-probability coupling $\Wt$ and therefore proves that Eq.~\eqref{eq:statemap} is a valid control refinement as formalized in Def.~\ref{def:validrefinement}. 
%		This concludes the proof of Thm.~\ref{thm:linear}.
%	}







\color{black}
\end{comment}


\section{Compositional approach for sub-probability couplings of two subsystems}
\Oliver{Insert short introduction with reference to \cite{lavaei2021compositional}.}\\
In the following, we drop the index $k$ on the time series $x_k,u_k$ for brevity.
Consider two gMDPs $\M_1(\theta_1),\M_2(\theta_2)$ with unknown parameters $\theta_1\in\Theta_1,\theta_2\in\Theta_2$, respectively:
\begin{align}
	\M_i(\theta_i): \left\{ \begin{array}{ll}
		\xp_i &= f_i(x_i,\left[u_i;\iin{i}\right];\theta_i)+ R_i w_i\\
		\left[y_{i};\iout{i}\right] &= h_i(x_i),
	\end{array} \right.\label{eq:nonlinear_sys_subsys_two}
\end{align}
where $\iin{i}\in\V_i\subseteq\Z_i$ denotes the internal input and $\iout{i}\in\Z_i$ the internal output of subsystem $i= 1,2$. Note that the output function can be decomposed as $h_i=\left[h_{i1};h_{i2}\right]$ such that $y_i=h_{i1}$ and $\iout{i}=h_{i2}$. The two subsystems are connected by setting $\iin{1}=\iout{2}$ and $\iin{2}=\iout{1}$.
The corresponding nominal models are given as
\begin{align}
	\Mh_i: \left\{ \begin{array}{ll}
		\xhp_i &= \hat f_i(\hat x_i, \left[\hat u_i;\iinh{i}\right];\theta^0_i)+ R_i\hat w_i\\
		\left[\hat y_{i};\iouth{i}\right] &=  \hat h_i( \hat x_i),
	\end{array} \right.\label{eq:nonlinear_nom_subsys_two}
\end{align}
where $\iinh{i}\in\Vh_i\subseteq\Z_i$ and $\iouth{i}\in\Z_i$, $i= 1,2$.
%The output $y_1$ of gMDP $\M_1$ consists of an external output $y_{11}$ and an internal output $y_{12}$, latter of which is used internally to connect $\M_1$ to $\M_2$ by setting $\iin{2}\equiv y_{12}$. We get $y_1:=[y_{11};y_{12}]$. The output of gMDPs $\M_2,\Mh_1,\Mh_2$ are defined analogously.

In the following, we assume that for both $i=1,2$ we have \mbox{$\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i$} and derive conditions so that \mbox{$\Mh\preceq^{\delta}_\eps\M$}, where $\Mh$ and $\M$ are the interconnections of their respective subsystems. We formalize these concepts mathematically next. First, we extend the definition of an SSR as stated in Def.~\ref{def:subsim} to subsystems.
\begin{definition}[SSR for subsystems]\label{def:ssr_subsys_two}
	%	\Oliver{Replacement for Def.~3.2 in \cite{lavaei2021compositional}.}
	Consider two gMDPs
	$\M\!=\!(\X,x_0,\A\times\V, \Tr, h, \Y\times\Z)$ and $\Mh\!=\!(\Xh,\xh{0},\Ah\times\Vh, \Trh, \hat h,  \Y\times\Z)$, measurable relations $\R_{x}\subset \Xh\times\X$ and $\R_{\iin{}}\subset \Vh\times\V$, and an interface function \(\InF :\Xh\times\X\times\Ah \rightarrow \A\). If there exists a sub-probability kernel  $\Wt(\cdot|\xh{},x, \red{(\uh{}, \iinh{}, \iin{})})$
	such that
	\begin{itemize}\itemsep=0pt
		\item[(a)] $(\hat x_{0}, x_{0})\in \R_{x}$;
		\item[(b)] for all $(\hat x,x)\in\R_{x}$, all $(\iinh{},\iin{})\in\R_{\iin{}}$, and $\ach{}\in \Ah$, $\Wt(\cdot|\xh{},x, \red{(\uh{}, \iinh{}, \iin{})})$ is a sub-probability coupling  of $\hat \Tr(\cdot|\hat x,\red{(\uh{}, \iinh{})})$ and $\Tr(\cdot|x,\red{(\InF, \iin{})})$ over $\R_{x}$ with respect to $\delta$ (c.f. Def.~\ref{def:submeasure_lifting}),
		\item[(c)] $\forall (\hat x,x)\in\R_{x}: \mathbf d_{\Y\times\Z}(\hat h(\hat x),h(x)) \leq \varepsilon$,
	\end{itemize}
	then $\Mh$ is in an $(\varepsilon,\delta)$-SSR with $\M$  that is denoted as \mbox{$\Mh\preceq^{\delta}_\eps\M$}.
\end{definition}

Next, we define the interconnection of multiple subsystems.

\begin{definition}[Interconnection of two subsystems]\label{def:interconnection_two}
	%	\Oliver{Replacement for Def.~4.1 in \cite{lavaei2021compositional}.}
	Consider two gMDPs $\M_i\!=\!(\X_i,x^0_i,\A_i\times\V_i, \Tr_i, h_i, \Y_i\times\Z_i)$, $i=1,2$, with an input-output configuration which can be partitioned as in \eqref{eq:nonlinear_sys_subsys_two}-\eqref{eq:nonlinear_nom_subsys_two}. Then, the \emph{interconnection} of the subsystems is a gMDP $\M\!=\!(\X,x^0,\A\times\V, \Tr, h, \Y\times\Z)$, also denoted as $\Interc{\M_1,\M_2}$, such that $\X=[\X_{1};\X_{2}]$, $\U=[\U_{1};\U_{2}]$, $\V=[\V_{1};\V_{2}]$, $\Y=[\Y_{1};\Y_{2}]$, $\Z=[\Z_{1};\Z_{2}]$, $h=[h_{11};h_{22}]$, with interconnection constraints
	\begin{align}
		\begin{split}\label{eq:interconnection_constraints_two}
			\iin{1}&=\iout{2},\; \Z_{2}\subseteq\V_{1}\\
			\iin{2}&=\iout{1},\; \Z_{1}\subseteq\V_{2}.
		\end{split}
	\end{align}
	The kernel and initial distribution are given as $\Tr=\Tr_{1}\Tr_2$ and $x^0=[x^0_{1};x^0_{2}]$, respectively.
\end{definition}

In the next theorem we establish \mbox{$\Mh\preceq^{\delta}_\eps\M$}, where $\M=\Interc{\M_1,\M_2}$ and $\Mh=\Interc{\Mh_1,\Mh_2}$, by induction from $\forall i=1,2:\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i$.


\begin{theorem}[\bfseries Induced compositional SSR]\label{thm:comp_induction_two}
	%	\Oliver{Replacement for Thm.~4.3 in \cite{lavaei2021compositional}.}
	Consider two gMDPs $\M_1(\theta_1),\M_2(\theta_2)$ forming an interconnected gMDP $\M(\theta)\!=\!(\X,x^0,\A\times\V, \Tr, h, \Y\times\Z)=\Interc{\M_1,\M_2}$, with $\theta:=[\theta_1,\theta_2]$. Suppose that there exist two corresponding abstract gMDPs $\Mh_1,\Mh_2$ independent of $\theta_1,\theta_2$, such that for both $i=1,2$ $\Mh_i$ is in an $(\varepsilon_i, \delta_i)$-SSR with $\M_i(\theta_i)$ as defined in Def.~\ref{def:ssr_subsys_two} with corresponding relations $R_{x_i}$, $\R_{\iin{i}}$, and sub-probability coupling $\Wt_i$. If we have
	\begin{align*}
		\forall (\hat x_1, x_1)\in\R_{x_1}&: \; \left(\hat h_{12}(\hat x_1), h_{12}(x_1)\right)\in\R_{\iin{2}}\\
		\forall (\hat x_2, x_2)\in\R_{x_2}&: \; \left(\hat h_{22}(\hat x_2), h_{22}(x_2)\right)\in\R_{\iin{1}},
	\end{align*}
%	\Oliver{(Note that indices of $h$ are different from \cite{lavaei2021compositional}.)}
	then $\Mh\!=\!(\Xh,\hat x^0,\Ah\times\Vh, \Trh, \hat h, \Y\times\Z)=\mathscr{I}(\Mh_1,\Mh_2)$ is in an \emph{induced compositional} $(\varepsilon, \delta)$-SSR with $\M(\theta)$ as defined in Def.~\ref{def:subsim} with a relation $\R$ given as 
	\begin{equation*}
		(\hat x, x)\in\R \Leftrightarrow \forall i=1,2:\; (\hat x_i, x_i)\in\R_{x_i}
	\end{equation*}
	where $\hat x:=[\hat x_1;\hat x_2]$ and $x:=[x_1;x_2]$,
	and $\varepsilon=\varepsilon_1+\varepsilon_2$, $\delta=1-(1-\delta_1)(1-\delta_2)$. Furthermore, we obtain the sub-probability coupling $\Wt=\Wt_{1}\Wt_2$ and the interface function $\InF=\InF_{1}\InF_2$, substituting with the interconnection constraints in \eqref{eq:interconnection_constraints_two}.
\end{theorem}
%\begin{proof}
%	See \ref{proof:linear_subsys_two}.
%\end{proof}

\subsection{Linear subsystems}
Let us now look at the case where the overall system can be decomposed into multiple linear subsystems $\M_i$. 
Consider $N$ interconnected gMDPs, $i=1,\ldots,N$, i.e.,
\begin{align}
	\M_i(\theta_i): \left\{ \begin{array}{ll}
		\xp_i &= A_i x_i+ B_i u_i+ D_i \iin{i}+ R_i w_i+F_i \theta_i\\
		y_i &= C_i x_i\\
		\iout{i} &= E_i x_i,
	\end{array} \right.\label{eq:linear_sys_subsys_two}
\end{align}
and corresponding nominal models
\begin{align}
	\Mh_i: \left\{ \begin{array}{ll}
		\xhp_i &= A_i \hat x_i+  B_i \hat u_i+ D_i \iinh{i}+ R_i\hat w_i\\
		\hat y_i &=  C_i \hat x_i\\
		\iouth{i} &= E_i \hat x_i.
	\end{array} \right.\label{eq:linear_nom_subsys_two}
\end{align}
The transition kernels can consequently be written as
\begin{align*}
	\Tr_i(\dxp_i \given x_i, u_i, \iin{i}) &= \mathcal N(\dxp_i|A_i x_i+ B_i u_i+ D_i \iin{i} +F_i \theta_i, R_iR_i\T)\\
	\Trh_i(\dxhp_i \given \hat x_i, \hat u_i, \iinh{i}) &= \mathcal N(\dxhp_i|A_i \hat x_i+ B_i \hat u_i+ D_i \iinh{i}, R_iR_i\T).
\end{align*}

%\hrule
We choose the interface function $\ac{i}\sim\InF_i(\cdot|\hat x_i, x_i, \hat u_i):=\ach{i}$,
and the noise coupling $\hat w_i=w_i+R^{-1}_i F_i\theta_i$ to get the state mapping
\[ \xhp_i = \xp_i-A (x_i-\hat x_i)-B (\ac{i}-\ach{i})-D(\iin{i}-\iinh{i}), \]
not dependent on $\theta$, i.e.,
\begin{equation}
	\label{eq:statemap_subsys_two}
	\xhp_i \sim \Refi_i(\cdot |\xh{i}, \x{i}, \xp_{i},\ach{i}) = \delta_{\xp_i-A x^\Delta_i-B u^\Delta_i-D\iin{i}^\Delta}(d\xhp_i),
\end{equation}
where $\iin{i}^\Delta:=\iin{i}-\iinh{i}$.
To establish an SSR $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$, we select the relations
\begin{align}
	\R_{x_i}&:=\{ (\hat x_i,x_i)\in\Xh_i\times\X_i \given x_i=\hat x_i\}\label{eq:R_x_two}\\
	\R_{\iin{i}}&:=\{ (\iinh{i},\iin{i})\in\Vh_i\times\V_i \given \iin{i}=\iinh{i}\}.\label{eq:R_v_two}
\end{align}
Condition (a) of Def.~\ref{def:ssr_subsys_two} holds by setting the initial states $\hat x^{0}_i = x^{0}_i$. Condition (c) is satisfied with $\eps_i=0$ since both systems use the same output mapping. For condition (b), we define the sub-probability coupling $\Wt_i$ of $\hat \Tr_i(\cdot|\hat x_i,\ach{i})$ and $\Tr_i(\cdot|x_i,\InF_i)$ over $\R_{x_i}$:
\begin{align}
	\begin{split}\label{eq:subprobcoup_subsys_two}
		\Wt_i
		&=\del{d\xhp_i}{\xp_i}
		\min\{\mathcal N(d\xp_i|\Phi_i,R_iR_i\T),\\&\mathcal N(d\xp_i|\Phi_i-R^{-1}_i F_i\theta_i, R_iR_i\T)\},
	\end{split}
\end{align}
with $\Phi_i := A_i x_i+ B_i u_i+ D_i \iin{i}+ F_i\theta_i$, that takes the minimum of two probability measures.

\begin{theorem}
	\label{thm:linear_subsys_two}
	For the linear models in \eqref{eq:linear_sys_subsys_two}-\eqref{eq:linear_nom_subsys_two}, we have that $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$ with interface function $\ac{i} = \ach{i}$, relations \eqref{eq:R_x_two}-\eqref{eq:R_v_two}, and the sub-probability kernel \eqref{eq:subprobcoup_subsys_two}. The state mapping \eqref{eq:statemap_subsys_two} defines a valid control refinement with $\eps_i=0$ and
	\begin{equation}
		\label{eq:delta_subsys_two}
		\delta_i = \sup_{\theta_i\in\Theta_i}\left\lbrace  1 - 2\cdot\cdf{-\frac{1}{2}\norm{R^{-1}_i F_i\theta_i}}\right\rbrace.
	\end{equation}
\end{theorem}
%\begin{proof}
%	See \ref{proof:linear_subsys_two}.
%\end{proof}

\subsection{Composed system}
Now we connect two subsystems, $i\in\{1,2\}$, with $\iin{1}=\iout{2}$ and $\iin{2}=\iout{1}$ (i.e., with $\iinh{1}=\iouth{2}$ and $\iinh{2}=\iouth{1}$). For $x:=[x_1,x_2]\T\in\X$, $\hat x:=[\hat x_1,\hat x_2]\T\in\Xh$, $u:=[u_1,u_2]\T\in\A$, $\hat u:=[\hat u_1,\hat u_2]\T\in\Ah$, and $\theta:=[\theta_1,\theta_2]\T\in\Theta$ we find the compositional transition kernels for the interconnected gMDPs $\M(\theta)$ and $\Mh$, namely
\begin{align*}
	\Tr(\dxp \given x, u) &= \mathcal N(\dxp|\bar A x+ B u+F \theta, RR\T)\\
	\Trh(\dxhp \given \hat x, \hat u) &= \mathcal N(\dxhp|\bar A \hat x+ B \hat u, RR\T).
\end{align*}
%with $u=\hat u$, $x=\hat x$, and 
where $B:=\mathrm{diag}(B_1,B_2)$, $F:=\mathrm{diag}(F_1,F_2)$, $R:=\mathrm{diag}(R_1,R_2)$, and
\begin{align*}
	\bar A&:=\begin{bmatrix} A_1 & D_1E_2 \\ D_2E_1 & A_2 \end{bmatrix}.
\end{align*}

We get the state mapping
\[ \xhp = \xp-\bar A (x-\hat x)-B (\ac{}-\ach{}), \]
not dependent on $\theta$, i.e.,
\begin{equation}
	\label{eq:statemap_comp_two}
	\xhp \sim \Refi(\cdot |\xh{}, \x{}, \xp{},\ach{}) = \delta_{\xp-\bar A x^\Delta-B u^\Delta}(d\xhp).
\end{equation}
To establish an SSR of the composed system, i.e., $\Mh\preceq^{\delta}_{\eps}\M(\theta)$, we select the relation
\begin{align}\label{eq:R_comp_two}
	\R_{x}&:=\{ (\hat x,x)\in\Xh\times\X \given x=\hat x\}
\end{align}
Condition (a) of Def.~\ref{def:subsim} holds by setting the initial states $\hat x^{0} = x^{0}$. Condition (c) is satisfied with $\eps=0$ since both compositional systems use the same output mapping, i.e., $C:=\mathrm{diag}(C_1,C_2)$. For condition (b), we define the sub-probability coupling $\Wt$ of $\hat \Tr(\cdot|\hat x,\ach{})$ and $\Tr(\cdot|x,\InF)$ over $\R_{x}$:
\begin{align}
	\begin{split}\label{eq:subprobcoup_comp_two}
		\Wt&=\del{d\xhp}{\xp} \min\{\mathcal N(d\xp|\Phi,RR\T),\\
		&\mathcal N(d\xp|\Phi-R^{-1}F\theta_, RR\T)\},
	\end{split}
\end{align}
with $\Phi := \bar A x+ B u+ F\theta$, that takes the minimum of two probability measures.

Now we want to establish a probabilistic relation after the composition using Thm.~\ref{thm:comp_induction_two}, which enables us to get guarantees on the closeness of the composed system and its abstraction using Thm.~\ref{thm:linear_subsys_two}.


\begin{theorem}
	Consider two pairs of linear subsystems \eqref{eq:linear_sys_subsys_two}-\eqref{eq:linear_nom_subsys_two}, where $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$ for $i=1,2$ with relations \eqref{eq:R_x_two}-\eqref{eq:R_v_two}, interface functions $u_i=\hat u_i$, and sub-probability kernels \eqref{eq:subprobcoup_subsys_two}.
	Let, $\M=\Interc{\M_1,\M_2}$ and $\Mh=\Interc{\Mh_1,\Mh_2}$ be the interconnections of these linear subsystems. Then Thm.~\ref{thm:comp_induction_two} holds, with relation $\R=\{ (\hat x,x)\in\Xh\times\X\given x=\hat x\}$, interface function $\ac{} = \ach{}$, and sub-probability kernel \eqref{eq:subprobcoup_comp_two}.
\end{theorem}
\begin{proof}
	It is trivial to show that the interconnection constraints in Thm.~\ref{thm:comp_induction_two} hold for this choice of $\R_{x_i},\R_{\iin{i}}$.
\end{proof}

\begin{remark}
	Limitations of the compositional approach ... \Oliver{TODO}
\end{remark}

==> fullLTL.tex <==
% !TEX root = main_cdc_22.tex
\color{blue}
\section{Expansion to full LTL}
Until now only addressed scLTL properties/specifications. Now we want to expand the method to approach the more expressive full LTL properties.
\begin{remark}[Finite-trace LTL (LTL\textsubscript{f})]
	%[\bfseries Finite-trace full LTL (LTL\textsubscript{f})}]
	The method described in this work is naturally applicable for full LTL specifications over finite-traces (LTL\textsubscript{f}) using the native approach outlined in \cite{Wells2020ftLTL}.
	LTL\textsubscript{f} semantics are particular useful for formalizing finite-horizon planning problems.
	With the approach in \cite{Wells2020ftLTL} our results for SSRs can be extended to LTL\textsubscript{f} by first translating the LTL\textsubscript{f} formula to an equivalent intermediate first-order logic (FOL) formula \cite{DeGiacomo2013ftLTL2FOL} and subsequently generating a minimal DFA using the tool MONA \cite{Henriksen1995MONA}.	
	Thereafter, the procedure remains the same, first constructing a product MDP and then solving the reachability problem (c.f. \cite{haesaert2020robust}).
	
%	Note that LTL\textsubscript{f} is expressively equivalent to FOL \cite{Kamp1968FOL2ftLTLequivalence}.
%	Furthermore, interesting extensions to dealing with more expressive monadic second-order logics (MSO) as in linear dynamic logics (LDL\textsubscript{f}) are addressed in \cite{Zhu2019LTLf2DFA}.
\end{remark}

However, one of the main strengths of our methods resides in the possibility of addressing infinite horizon specifications. This motivates us to extend the approach to infinite-trace LTL as well. For this, we approximate the repeated reachability using the method outlined in \cite{kazemi2020fullLTL}.
\newline

%From the results of the previous sections we have
%\begin{equation*}
%	\P\left(\Ca \times \M(\theta) \satisfies \psi_{scLTL} \right)\geq   p_{\psi_{scLTL}}, \quad  \forall \theta\in\Theta.
%\end{equation*}
%We now want to expand this to full LTL specifications, i.e.,
%\begin{equation*}
%	\P\left(\Ca \times \M(\theta) \satisfies \psi_{LTL} \right)\geq   p_{\psi_{LTL}}, \quad  \forall \theta\in\Theta.
%\end{equation*}
%
%From \cite{kazemi2020fullLTL} we have
%\begin{equation*}
%	p_l \leq \sup_{\Ca}\,\P\left(\Ca \times \M(\theta) \satisfies \psi_{LTL} \right) \leq p_u, \quad  \forall \theta\in\Theta,
%\end{equation*}
%where the upper and lower bounds are given by
%\begin{align*}
%	p_u &:= \sup_{\boldsymbol{\mu}}\,\P\left(\boldsymbol{\mu} \times \left(\M(\theta) \times \tilde{\mathcal{A}}_\psi\right)_\zeta \satisfies \Event\phi \right)\text{, and}\\
%	p_l &:= 1-\sup_{\boldsymbol{\mu}}\,\P\left(\boldsymbol{\mu} \times \left(\M(\theta) \times \tilde{\mathcal{A}}_{\notltl\psi}\right)_\zeta \satisfies \Event\phi \right).
%\end{align*}
%Here, $\Ca$ is a finite-memory control strategy \Oliver{(Check whether definition in Sec.~\ref{sec:MDPs} is valid for this (freedom to use LDBA instead of DFA?!))}, whereas $\boldsymbol{\mu}$ is a Markov policy. Furthermore, $\tilde{\mathcal{A}}_\psi$ is a LDBA for specification $\psi$.

\begin{align*}
	\notag \textstyle \mathbf T_{}^{\mu} (V)(\hat x,q)\!:=\!&\int_{\Xh\times Q} \max\left\{\mathbf 1_{F}(q'), V(\hat x',q')\right\}\\ &\times \Trh(d \hat x'| \hat x,\mu) \times \bar\trans(q'|q,\hat x')
\end{align*}

We get 
\begin{align*}
	\mathbf T_{}^{\mu} (V)(\hat x,q)\!:=\!
	\begin{cases}
		1 \text{, for $(\hat x,q)=\phi$}\\
		(1-\xi)+\xi \int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x') \text{, for $(\hat x,q)\in F$}\\
		\int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x') \text{, otherwise}
	\end{cases}
\end{align*}
with $\bar\trans(q,\hat x'):=\{\trans(q,\alpha)\mbox{ with }\alpha \in\Lab(B_\varepsilon( \hat h (\hat x')))\}$.
%Since the integral term is upper bounded by one, the term in the second case is always greater or equal to the third one and hence we can write
%\begin{align*}
%	&\mathbf T_{}^{\mu} (V)(\hat x,q)\!:=\!\\
%	&\int_{\Xh\times Q} \max\left\{\1_{\phi}(\hat x, q), \1_{F}(\hat x, q)(1-\xi)+\xi \int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x'), \int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x')\right\}
%\end{align*}
We define the $\delta$-robust operator
\begin{align*}
	\mathbf T_{\delta}^{\mu} (V)(\hat x,q)\!:=\!\Lim\left(
	\begin{cases}
		1-\delta \text{, for $(\hat x,q)=\phi$}\\
		(1-\xi)+\xi \int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x')-\delta \text{, for $(\hat x,q)\in F$}\\
		\int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x')-\delta \text{, otherwise}
	\end{cases}\right) 
\end{align*}
and the optimal $\delta$-robust operator
\begin{align*}
	\mathbf T_{\delta}^{\ast} (V)(\hat x,q)\!:=\!\sup_{\mu}\Lim\left(
	\begin{cases}
		1-\delta \text{, for $(\hat x,q)=\phi$}\\
		(1-\xi)+\xi \int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x')-\delta \text{, for $(\hat x,q)\in F$}\\
		\int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu) \times \bar\trans(q'|q,\hat x')-\delta \text{, otherwise}
	\end{cases}\right) 
\end{align*}

For the optimal $(\varepsilon,\delta)$-robust operator we get
\begin{align*}
	\notag \textstyle \mathbf T_{\eps,\delta}^{\ast} (V)(\hat x,q)\!:=\!
	\sup_{\mu}\Lim\left( \!\!\int_{\hat\X} \min_{q'\in \bar\trans(q,\hat x')}\!\!\
	\begin{cases}
		1-\delta \text{, for $(\hat x,q)=\phi$}\\
		(1-\xi)+\xi \int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu)-\delta \text{, for $(\hat x,q)\in F$}\\
		\int_{\Xh\times Q}V(\hat x',q') \times \Trh(d\hat x'|\hat x,\mu)-\delta \text{, otherwise}
	\end{cases}\right)
\end{align*}
which takes the worst-case location $q'$ considering an $\varepsilon$-ball around the systems output $\hat h (\hat x')$ as described earlier.
\newpage
.
\newpage
\color{black}

==> nonlinear_apprx.tex <==
% !TEX root = main_cdc_22.tex
Consider two bounds. One bound on the step by step deviation that can be caused by the unknown parameter, and one deviation that is caused by state discrepancies between the two models. 
Let us assume that for the former, we can bound it as
\begin{align}
\|	f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)\|\leq d.
\end{align}

We can rewrite the original model as follows:
\begin{align*}
	x_{k+1} &=\underbrace{f(x_k, u_k;\theta_0)}_{nominal dynamics} + \underbrace{ f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)+w_k}_{disturbance}.
\end{align*}

We can now start relating the stochastic models by coupling over a subset where the disturbances are equal, that is, we search for a sub-probability coupling $\bar{\mathbf{w}}$ for which $\support(\bar{\mathbf{w}})\subset \{f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)+w_k= \hat w_k\}$. 

This leads to a sub-probability kernel $\Wt$ that is similar to the kernel \eqref{eq:ex_v} in   Example \ref{ex:lineartheta}, and that is hence similarly based on a sub-probability coupling \eqref{eq:ex_w}. 
If we look at the behaviour of the two stochastic systems constrained to $  \{f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)+w_k= \hat w_k\}$, we have that  
\begin{align*} 
		\hat x_{k+1} &=   f(\hat x_{k},\hat u_k; \theta_0)+  \hat  w_k\\
		x_{k+1} &=f(x_k, u_k;\theta_0) + \underbrace{ f(x_k, u_k;\theta)-f(x_k, u_k;\theta_0)+w_k}_{=\hat w_k}.
\end{align*}
Furthermore, the error dynamics $\Delta x_k:= 	x_{k}-\hat x_k $ evolve as
 \begin{align*} 
\Delta	x_{k+1} &=f(x_k, u_k;\theta_0) -   f(\hat x_{k},\hat u_k; \theta_0).
\end{align*}
As an update relation we get
\begin{equation}
	\hat x_{k+1} = x_{k+1} + f(\hat x_{k},\hat u_k; \theta_0) - f(x_k, u_k;\theta_0).
\end{equation}

==> partial_RFF.tex <==
%!TeX root=main_cdc_22.tex

\begin{figure}[htp]
	\centering
	\scalebox{0.9}{	\begin{tikzpicture}
			


			\node[draw,rectangle, fill=gray!50, node distance=6.5cm] (M2) {\begin{minipage}[c]{3.3cm}
					\begin{align*}\SwapAboveDisplaySkip
						\M
					\end{align*}
				\end{minipage}
			};
			
			\node[above of =M2,draw ,rectangle, anchor=south west,fill=lightyellow, node distance=1.6cm] (if2) {\begin{minipage}[c]{2cm}
					Interface
					\begin{align*}\SwapAboveDisplaySkip
						\InF 
					\end{align*}
				\end{minipage}
			};
			\node[above of =M2, draw,rectangle, anchor=south east,fill=lightyellow, node distance=1.6cm] (lif2) {\begin{minipage}[c]{2cm}
					Refinement 
					\begin{align*}\SwapAboveDisplaySkip
					\Refi	\end{align*}
				\end{minipage}
			};
			\path[draw] (if2.south) edge[latex-,right] node{$\x{k} $}(if2.south |- M2.north);
			
			\node[right of =M2, node distance= 3cm](out2){$\y{k}$};
			
			\path[draw] (lif2.south) ++(-0.5cm,0)  edge[latex-,left] node{$ \x{k+1}$} ([xshift=-0.5cm]lif2.south |- M2.north);
			\path[draw] (lif2.south) ++(-0cm,0)  edge[latex-,right] node{$ \x{k}$} ([xshift=-0cm]lif2.south |- M2.north);
			\path[draw] (if2.south) ++(-0.5cm,0)  edge[-latex,left] node{$\ac{k}$} ([xshift=-0.5cm]if2.south |- M2.north);
			
			\node[left of =M2, node distance=2cm,yshift=4cm](MM2) {$\Ca$};
			\node[above of =M2,draw,fill=gray!15, rectangle, minimum width=3.3cm,node distance=5cm, minimum height=1cm] (Ca2) {$\widehat{\Ca}$};
			\path[draw] (Ca2.south) ++(-0.25cm,0)  edge[-latex,right]node{$ \ach{k}$} ([xshift=-0.25cm]Ca2.south |- if2.north);
			\path[draw] (Ca2.south) ++(-1.25cm,0)  edge[latex-,left] node{$ \xh{k+1}$} ([xshift=-1.25cm]Ca2.south |- if2.north);
			\path[draw] (Ca2.south) ++(-.85cm,0)  edge[-latex,right] node{$ \xh{k}$} ([xshift=-.85cm]Ca2.south |- if2.north);
			\path[draw] (Ca2.south) ++(0.5cm,0)  edge[-latex,right] node{$ \ach{k}$} ([xshift=0.5cm]Ca2.south |- if2.north);
			\path[draw] (Ca2.south) ++(1cm,0)  edge[-latex,right] node{$ \xh{k}$} ([xshift=1cm]Ca2.south |- if2.north);
			\begin{scope}[on background layer]
				
				\node[ fill=gray!40, fit= (MM2)(if2)(lif2)(Ca2)](FIt1) {};
				\path[draw] (M2) edge[-latex] (out2);
				
			\end{scope}
		\end{tikzpicture}
	}
	
	
	\caption{Using the conditional lifting for control refinement.  }
	\label{fig:aux_model_3}
\end{figure}
